Surface Defect Identification using Bayesian Filtering on a 3D Mesh

This paper presents a CAD-based approach for automated surface defect detection. We leverage the a-priori knowledge embedded in a CAD model and integrate it with point cloud data acquired from commercially available stereo and depth cameras. The proposed method first transforms the CAD model into a high-density polygonal mesh, where each vertex represents a state variable in 3D space. Subsequently, a weighted least squares algorithm is employed to iteratively estimate the state of the scanned workpiece based on the captured point cloud measurements. This framework offers the potential to incorporate information from diverse sensors into the CAD domain, facilitating a more comprehensive analysis. Preliminary results demonstrate promising performance, with the algorithm achieving convergence to a sub-millimeter standard deviation in the region of interest using only approximately 50 point cloud samples. This highlights the potential of utilising commercially available stereo cameras for high-precision quality control applications.

==> Abstract/abstract-content.tex <==
Industry 4.0 relies on the circular dependency between data collected
from the process and their exploitation to adapt and improve the
production rate and variety~\cite{Catalucci2022}.  In this context,
automatic defect detection in industrial production and assembly lines
is paramount for delivering products that match the continuously
growing quality requirements.  In particular, one of the main open
issues in the automotive industry is the identification of small
defects on metallic surfaces that are due to welding operations (weld
splatters) or other mechanical processes (dents).

Even though the task of detecting anomalies is repetitive in the
automotive sector, it is still performed manually due to the
complexity of the problem.  To automate this task, research focused on
2D vision systems.  Promising results are from deflectometry, an
optical based method which measures the deformation patterns of
structured light~\cite{ARNAL2017306,MOLINA2017263}.  This method
however requires high reflectance to properly work, thus only painted
vehicles can be used.  Considering that a significant amount of
defects could be revealed right after weld and assembly processes,
their immediate recognition can reduce the required rework time.

Defects are identified in images leveraging machine learning methods
that, despite their encouraging performance in structured
environments~\cite{Chang2019}, lack generalisation to different
products and scenarios, limiting their exploitation in flexible
production processes~\cite{Lehr2021}. On the other hand, a rich source
of information that is always available is the CAD model of the
workpiece.  This knowledge is mainly used for geometric tolerance
inspection~\cite{Sjodahl_2021}, while little research compared the CAD
with 3D point cloud measurements to classify different
defects~\cite{Doring2006}.

In this paper we address the surface defect detection problem by
combining the CAD model knowledge with several point cloud
measurements acquired through commercially available stereo cameras.
The CAD is represented by a high-density polygonal mesh.  We assign to
each vertex a degree of freedom that encodes the surface state.  In
virtue of this representation, the weighted least squares estimator
fuses point cloud measurements in order to effectively reconstruct the
workpiece mesh starting from the prior knowledge provided by the CAD.
Once the surface state is estimated, defect segmentation is carried
out by measuring spatial correlation between close vertices.
In the final setup, the camera will be mounted on a robotic manipulator in order to provide full coverage of the workpiece.

In this preliminary work, we evaluate the accuracy and convergence
features of the detection algorithm using a 3D-printed plastic board
with a known defect shape.  Point cloud measurements are collected
from two commercial cameras for comparison: the Intel RealSense D415 and
the StereoLabs ZED2.  We consider a static environment with the
relative pose between camera and workpiece provided by a motion
capture system and acting as a ground truth reference.  The results of
the experiments, which characterise the minimum perceivable defect of
the different systems as well as its computational time, will show the
limits of the applicability of the method for the task at hand.


==> Makefile <==
# Makefile for LaTeX files

LATEX	= pdflatex
BIBTEX	= bibtex
MAKEINDEX = makeindex

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"
MAKEIDX = "^[^%]*\\makeindex"
MAKETOC = "^[^%]*\\tableofcontents"
MPRINT = "^[^%]*print"
USETHUMBS = "^[^%]*thumbpdf"

SRC	:= $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex)
BIBFILE := $(shell perl -ne '($$_)=/^[^%]*\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $(SRC))

PDFPICS := $(shell perl -ne '@foo=/^[^%]*\\(includegraphics)(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.pdf$$/) { print "$$foo[2] "; } else { print "$$foo[2].pdf "; }}' *.tex)
DEP	= *.tex

TRG	= $(SRC:%.tex=%.pdf)

COPY = if test -r $(<:%.tex=%.toc); then cp $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); fi 
RM = rm -f
OUTDATED = echo "EPS-file is out-of-date!" && false


all 	: $(TRG)

define run-latex
	  $(COPY);$(LATEX) $<
	  egrep -q $(MAKEIDX) $< && ($(MAKEINDEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) ; true
	  egrep -q $(MAKETOC) $< && ($(MAKEINDEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) ; true
	  egrep -c $(RERUNBIB) $(<:%.tex=%.log) && ($(BIBTEX) $(<:%.tex=%);$(COPY);$(LATEX) $<) ; true
	  egrep -q $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) ; true
	  egrep -q $(RERUN) $(<:%.tex=%.log) && ($(COPY);$(LATEX) $<) ; true
	  if cmp -s $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); then true ;else $(LATEX) $< ; fi
	  $(RM) $(<:%.tex=%.toc.bak)
	  # Display relevant warnings
	  egrep -i "(Reference|Citation).*undefined" $(<:%.tex=%.log) ; true
endef

$(TRG)	: %.pdf : %.tex $(DEP) $(PDFPICS) $(BIBFILE)
	  @$(run-latex)

clean	:
	  -rm -f $(TRG) $(PSF) $(PDF) $(TRG:%.pdf=%.aux) $(TRG:%.pdf=%.bbl) $(TRG:%.pdf=%.blg) $(TRG:%.pdf=%.log) $(TRG:%.pdf=%.out)

.PHONY	: all show clean ps pdf showps

view:
	acroread $(PDF)

osx:
	open $(PDF)

######################################################################
# Define rules for PDF source files.
%.pdf: %.eps
	epstopdf $< > $(<:%.eps=%.pdf)


==> Sections/relatedworks.tex <==
\section{Related works}
\label{sec:relatedworks}


